A Tandem Framework Balancing Privacy and Security for Voice User Interfaces

Speech synthesis, voice cloning, and voice conversion techniques present severe privacy and security threats to users of voice user interfaces (VUIs). These techniques transform one or more elements of a speech signal, e.g., identity and emotion, while preserving linguistic information. Adversaries may use advanced transformation tools to trigger a spoofing attack using fraudulent biometrics for a legitimate speaker. Conversely, such techniques have been used to generate privacy-transformed speech by suppressing personally identifiable attributes in the voice signals, achieving anonymization. Prior works have studied the security and privacy vectors in parallel, and thus it raises alarm that if a benign user can achieve privacy by a transformation, it also means that a malicious user can break security by bypassing the anti-spoofing mechanism. In this paper, we take a step towards balancing two seemingly conflicting requirements: security and privacy. It remains unclear what the vulnerabilities in one domain imply for the other, and what dynamic interactions exist between them. A better understanding of these aspects is crucial for assessing and mitigating vulnerabilities inherent with VUIs and building effective defenses. In this paper,(i) we investigate the applicability of the current voice anonymization methods by deploying a tandem framework that jointly combines anti-spoofing and authentication models, and evaluate the performance of these methods;(ii) examining analytical and empirical evidence, we reveal a duality between the two mechanisms as they offer different ways to achieve the same objective, and we show that leveraging one vector significantly amplifies the effectiveness of the other;(iii) we demonstrate that to effectively defend from potential attacks against VUIs, it is necessary to investigate the attacks from multiple complementary perspectives(security and privacy).

==> reconstruction_attack.tex <==
\section{Reconstruction Attack}
\label{sec:reconstruction_attack}

Let $F_\theta$ denote a neural network with parameters $\theta$. The function inputs and outputs have the same dimension as the target embedding x, x $\in$ $R^d$, $\in$ $F_\theta(x)$ $\in$ $R^d$.

Inspired by Siamese Network, we develop two identical, weight-shared, instances of $F_\theta$. We then use the cosine similarity between the reconstructed embedding of two given inputs, setting the target value to 1 if the two input low-quality embeddings belong to the same data point, and 0 otherwise. Formally, let $x_1^{row}$ , $x_2^{row}$ denote two row data sample $d_1$, $d_2$ respectively and $x_1^{anon}$,$x_2^{anon}$ their anonymized counterparts. We train $F_\theta$ using a summation of the two reconstruction losses and the cosine similarity loss denoted by L:

\begin{equation}
L = \left \| F_\theta (x_1^{anon}) - x_1^{row} \right \|^2 + \left \| F_\theta (x_2^{anon}) - x_2^{row} \right \|^2 
\end{equation}

\begin{equation}
\frac{F_\theta (x_1^{anon})  \cdot F_\theta (x_2^{anon})}{ \left \| F_\theta (x_1^{anon})\right \|   \left \| F_\theta (x_2^{anon}\right \| } -  \delta_{d_1,d_2}
\end{equation}

Where,
\begin{equation}
\delta_{d_1,d_2} = 
    \begin{cases}
      1, & \text{if}\ d_1 = d_2 \\
      0, & \text{otherwise}
    \end{cases}
\end{equation}

To reconstruct an embedding during inference, one simply uses the output of $F_\theta$ without using the Siamese training scheme.

Assuming that we have recordings of the target speaker which are publicly available, then the 
\textbf{Potential Attacks on Anonymized Recordings:}
\begin{itemize}
\item Siamese x-vector Reconstruction~\cite{rozenberg2020siamese, hajavi2020siamese}: under three mismatch scenarios: noise, sampling rate, and telephone simulation. The anonymized/converted recordings may suffer from one of these conditions (\ie~embedding reconstruction)-distribution mismatch problem.
\item Membership Attacks~\cite{hisamoto2020membership}: given a model and an anonymized record, determine whether this record was used as part of the model’s training dataset or not (\ie~enrollment stage)
\end{itemize}

